Leave-One-Out Cross-Validation for Bayesian Model Comparison in Large Data

Recently, new methods for model assessment, based on subsampling and posterior approximations, have been proposed for scaling leave-one-out cross-validation (LOO) to large datasets. Although these methods work well for estimating predictive performance for individual models, they are less powerful in model comparison. We propose an efficient method for estimating differences in predictive performance by combining fast approximate LOO surrogates with exact LOO subsampling using the difference estimator and supply proofs with regards to scaling characteristics. The resulting approach can be orders of magnitude more efficient than previous approaches, as well as being better suited to model comparison.

==> tables/fig_table_blr1000.tex <==
\begin{table}[ht]
\begin{minipage}[t]{0.52\linewidth}
\centering
\caption{Comparing BLR models with different number of included covariates with $m=100$ and the difference estimator and plpd as approximation. The true model is $D=100$.} \label{tab:model_compare_blr1000}
\begin{tabular}{lrrrr}
  \toprule
Model & $\widehat{\text{elpd}}_\text{D}$ & SE($\widehat{\text{elpd}}_\text{D}$) & $\hat{\sigma}_{D}$ & $\widehat{\text{elpd}}_\text{M}$ \\ 
  \midrule
  $D=100$ & 0.0 & 0.0 & 0.0 & -48945 \\ 
  $D=90$ & -48.9 & 1.4 & 11.8 & -48994 \\ 
  $D=99$ & -11.8 & 0.9 & 5.1 & -48957 \\ 
  $D=101$ & -2.1 & 0.8 & 0.6 & -48947 \\
  $D=110$ & -6.1 & 1.4 & 3.4 & -48951 \\ 
  \bottomrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[t]{0.44\linewidth}
\centering
 % Caption and label go in the first argument and the figure contents
 % go in the second argument
  \captionof{figure}{1000 estimates of $\sigma_\text{loo}$ for Radon Model 6 using $\text{WAIC}_{2k}$ for $\tilde{\pi}$. True value is 96.} 
  {\includegraphics[width=1\linewidth]{images/sigma_est.png}}
  \label{fig:sigma_est}
\end{minipage}
\end{table}


==> tables/table_approx_tilde.tex <==
\begin{table}
  \caption{Approximations for $\tilde{\pi}$ and their computational costs}
  \label{tab:approx_tilde}
  \centering
  \begin{tabular}{lll}
    \toprule
%    \multicolumn{2}{c}{Part}                   \\
%    \cmidrule(r){1-2}
    Approximation     & Needs     & Cost \\
    \midrule
    plpd & $\hat{\theta}$ & $O(nP)$     \\
    $\text{WAIC}_\text{S}$ & $S$ draws from $p(\theta|y)$  & $O(nPS)$     \\
    $\text{TIS}_\text{S}$ & $S$ draws from $p(\theta|y)$  & $O(nPS)$     \\    
    $\Delta_1\text{WAIC}_\text{m}$ & $\nabla \log p(y_i|\theta)$, $\hat{\theta}$ and $\text{tr}(\Sigma_{\theta})$ & $O(nP)$  \\    
    $\Delta_1\text{WAIC}$ & $\nabla \log p(y_i|\theta)$, $\hat{\theta}$ and $\Sigma_{\theta}$ & $O(nP^2)$     \\
    $\Delta_2\text{WAIC}$  & $\nabla \log p(y_i|\theta)$, $H_\theta$, $\hat{\theta}$ and $\Sigma_{\theta}$ & $O(nP^3)$     \\
    \bottomrule
  \end{tabular}
\end{table}



==> tables/table_big_compare_tis.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Thu May 23 10:12:11 2019
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
  \toprule
post\_name & elpd\_diff\_hat & se\_elpd\_diff\_hat & se\_diff\_hat & elpd\_loo\_hat \\ 
  \midrule
HS & 0 & 0 & 0 & -372348 \\ 
  N & -47.6 & 5.150 & 8.8 & -372395 \\ 
  N & -52.3 & 0.035 & 8.8 & -372401 \\ 
  \midrule
HS & 0 & 0 & 0 & -3721821 \\ 
  N & -44.7 & 7.021 & 9 & -3721865 \\ 
  N & -49.3 & 0.040 & 9 & -3721871 \\ 
   \bottomrule
\end{tabular}
\caption{Comparing a Normal prior (N) with a horseshoe prior for 1M and 100k observations using a subsampling size of m=100 and the diference estimator.} 
\label{tab:big_compare}
\end{table}

==> tables/table_hh_vs_diff.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Fri May 17 10:01:49 2019
\begin{table}[ht]
\caption{Difference vs. Hansen-Hurwitz estimation using a subsampling size of $m=100$. Posteriors has been computed using MCMC and the results are averaged over 100 repetitions, standard error over repetitions in parenthesis.} 
\label{tab:hh_vs_diff}
\centering
\begin{tabular}{lrrrrrrrrr}
  \toprule
Data & Model & SE($\widehat{\text{elpd}}_\text{diff,WAIC}$) & SE($\widehat{\text{elpd}}_\text{HH,WAIC}$) & Ratio \\ 
  \midrule
Radon & 1 & 0.002 (0.00) & 0.001 (0.00) & 1.47 \\ 
   & 2 & 1.037 (0.09) & 0.809 (0.08) & 1.28  \\ 
   & 3 & 9.203 (1.84) & 6.375 (1.13) & 1.44  \\    
   & 4 & 0.954 (0.12) & 0.786 (0.06) & 1.21  \\ 
  & 5 & 13.277 (2.90) & 12.443 (1.81) & 1.07  \\   
   & 6 & 10.339 (1.90) & 14.536 (1.70) & 0.71 \\ 
  \midrule   
  $R^2=0.9$ & BLR  & 0.034 (0.00) & 0.023 ( 0.00) & 1.47 \\ 
  $R^2=0.5$ &  & 0.036 (0.00) & 0.027 ( 0.00) & 1.35 \\ 
  $R^2=0.1$ &  & 0.039 (0.00) & 0.030 ( 0.00) & 1.29  \\ 
   \bottomrule
\end{tabular}
\end{table}


==> tables/table_model_compare_bigcompare.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Thu May 16 10:32:30 2019
\begin{table}[ht]
\centering
\caption{Comparing priors using a subsample of size $m=100$ using the difference estimator and the WAIC as approximation and a Horseshoe (HS) and Normal (N) priors.}
\label{tab:model_compare_bigcompare}
\begin{tabular}{llrrrr}
  \toprule
$n$ & Prior & $\widehat{\text{elpd}}_\text{D}$ & SE($\widehat{\text{elpd}}_\text{D}$) & $\hat{\sigma}_{D}$ & $\widehat{\text{elpd}}_\text{M}$ \\ 
  \midrule
  0.1M & HS & 0.0 & 0.0 & 0.0 & -372349 \\
  & N & -52.3 & 0.0 & 8.8 & -372401 \\  
  1M & HS & 0.0 & 0.0 & 0.0 & -3721822 \\
  & N & -49.2 & 0.0 & 9.0 & -3721871 \\
   \bottomrule
\end{tabular}
\end{table}

==> tables/table_model_compare_blr0010.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Mon May 13 21:49:15 2019
\begin{table}[ht]
\centering
\caption{Comparing models using a subsampling size of m=100 using the difference estimator and the waic as approximation. Posteriors has been computed using MCMC.} 
\begin{tabular}{lrrrr}
  \toprule
post\_name & elpd\_diff\_hat & se\_elpd\_diff\_hat & se\_diff\_hat & elpd\_loo\_hat \\ 
  \midrule
blrD100 & 0.0 & 0.0 & 0.0 & -25751.0 \\
  blrD110 & -2.1 & 0.0 & 3.9 & -25753.2 \\ 
  blrD101 & -0.2 & 0.0 & 1.5 & -25751.3 \\ 
  blrD099 & -432.7 & 0.0 & 28.8 & -26183.8 \\ 
  blrD090 & -3510.9 & 0.0 & 70.9 & -29262.0 \\ 
   \bottomrule
\end{tabular}

\label{tab:model_compare_blr0010}
\end{table}

==> tables/table_model_compare_blr0100.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Mon May 13 21:55:52 2019
\begin{table}[ht]
\centering
\caption{Comparing models using a subsampling size of m=100 using the difference estimator and the waic as approximation. Posteriors has been computed using MCMC.} 
\begin{tabular}{lrrrr}
  \toprule
post\_name & elpd\_diff\_hat & se\_elpd\_diff\_hat & se\_diff\_hat & elpd\_loo\_hat \\ 
  \midrule
  blrD100 & 0.0 & 0.0 & 0.0 & -37142 \\
  blrD110 & -1.1 & 0.0 & 4.1 & -37143 \\ 
  blrD101 & -0.3 & 0.0 & 0.4 & -37142 \\ 
  blrD099 & -50.2 & 0.0 & 9.9 & -37192 \\
  blrD090 & -504.9 & 0.0 & 31.6 & -37647 \\ 
   \bottomrule
\end{tabular}
\label{tab:model_compare_blr0100}
\end{table}

==> tables/table_model_compare_radon_100.tex <==

% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Mon May 13 20:51:19 2019
\begin{table}[ht]
\centering
\caption{Comparing models using a subsample of size $m=100$ using the difference estimator and the WAIC as approximation.} 
\label{tab:model_compare_radon_100}
\begin{tabular}{lrrrr}
  \toprule
$M$ & $\widehat{\text{elpd}}_\text{D}$ & SE($\widehat{\text{elpd}}_\text{D}$) & $\hat{\sigma}_{D}$ & $\widehat{\text{elpd}}_\text{M}$ \\ 
  \midrule
6 & 0.0 & 0.0 & 0.0 & -16854.1 \\ 
  5 & -1424.1 & 34.4 & 51.7 & -18278.2 \\ 
  4 & -168.0 & 53.6 & 27.4 & -17022.1 \\ 
  3 & -307.6 & 91.6 & 29.6 & -17161.7 \\ 
  2 & -234.7 & 53.6 & 28.2 & -17088.9 \\ 
  1 & -1705.4 & 53.7 & 58.9 & -18559.5 \\ 
   \bottomrule
\end{tabular}
\end{table}



==> tables/table_model_compare_radon_400.tex <==

% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Thu May 16 17:20:41 2019
\begin{table}[ht]
\centering
\caption{Comparing Radon models using a subsample of size of $m=400$ using the difference estimator and WAIC as approximation.} 
\label{tab:model_compare_radon_400}
\begin{tabular}{lrrrr}
  \toprule
$M$ & $\widehat{\text{elpd}}_\text{D}$ & SE($\widehat{\text{elpd}}_\text{D}$) & $\hat{\sigma}_{D}$ & $\widehat{\text{elpd}}_\text{M}$ \\ 
  \midrule
6 & 0.0 & 0.0 & 0.0 & -16807.2 \\ 
  5 & -1451.8 & 8.9 & 51.5 & -18258.9 \\ 
  4 & -215.0 & 13.4 & 26.2 & -17022.2 \\ 
  3 & -281.8 & 22.6 & 27.9 & -17088.9 \\ 
  2 & -282.1 & 13.4 & 28.1 & -17089.2 \\   
  1 & -1752.4 & 13.4 & 58.2 & -18559.5 \\ 
   \bottomrule
\end{tabular}
\end{table}


==> tables/table_performance.tex <==
% latex table generated in R 3.5.1 by xtable 1.8-3 package
% Fri May 17 10:01:49 2019
\begin{table}[ht]
\caption{Different subsampling approaches to estimate $\text{elpd}_\text{loo}$ using a subsampling size of $m=100$. Posteriors has been computed using MCMC and the results are averaged over 100 runs with standard errors over runs in parenthesis.} 
\label{tab:performance}
\centering
\begin{tabular}{lrrrrrrrrr}
  \toprule
Data & Model & SE($\widehat{\text{elpd}}_\text{diff,WAIC}$) & SE($\widehat{\text{elpd}}_\text{HH,lpd}$) & Ratio & SE($\widehat{\text{elpd}}_\text{SRS}$) & $\hat{\sigma}_\text{elpd}$ \\ 
  \midrule
Radon & 1 & 0.002 (0.00) & 0.7 (0.03) & 0.003 & 949 (20) & 88 \\ 
   & 2 & 1.037 (0.09) & 41.6 (0.81) & 0.025 & 1012 (23) & 94 \\ 
   & 3 & 9.203 (1.84) & 74.4 (4.95) & 0.124 & 1012 (23) & 94 \\    
   & 4 & 0.954 (0.12) & 40.1 (0.78) & 0.024 & 1013 (23) & 94 \\ 
  & 5 & 13.277 (2.90) & 84.3 (7.22) & 0.158 & 972 (19) & 90 \\   
   & 6 & 10.339 (1.90) & 97.2 (6.93) & 0.106 & 1050 (24) & 96 \\ 
  \midrule   
  $R^2=0.9$ & BLR  & 0.034 (0.00) & 4.0 (0.04) & 0.009 & 704 (11) & 70 \\ 
  $R^2=0.5$ &  & 0.036 (0.00) & 4.9 (0.04) & 0.007 & 711 (14) & 72 \\ 
  $R^2=0.1$ &  & 0.039 (0.00) & 5.8 (0.07) & 0.007 & 756 (13) & 76 \\ 
   \bottomrule
\end{tabular}
\end{table}



==> tables/table_radon_models_approx_tilde.tex <==
\begin{table}[ht]
    \begin{minipage}[t]{.6\linewidth}
  \caption{Computational costs for approximations of $\pi$ }
  \label{tab:approx_tilde}
  \centering
  \begin{tabular}{lll}
    \toprule
%    \multicolumn{2}{c}{Part}                   \\
%    \cmidrule(r){1-2}
    $\tilde{\pi}$     & Needs     & Cost \\
    \midrule
    plpd & $\hat{\theta}$ & $O(nP)$     \\
    $\text{WAIC}_\text{S}$ & $S$ draws from $p(\theta|y)$  & $O(nPS)$     \\
    $\text{TIS}_\text{S}$ & $S$ draws from $p(\theta|y)$  & $O(nPS)$     \\    
    $\Delta_1\text{WAIC}_\text{m}$ & $\nabla \log p(y_i|\theta)$, $\hat{\theta}$ and $\text{tr}(\Sigma_{\theta})$ & $O(nP)$  \\    
    $\Delta_1\text{WAIC}$ & $\nabla \log p(y_i|\theta)$, $\hat{\theta}$ and $\Sigma_{\theta}$ & $O(nP^2)$     \\
    $\Delta_2\text{WAIC}$  & $\nabla \log p(y_i|\theta)$, $H_\theta$, $\hat{\theta}$ and $\Sigma_{\theta}$ & $O(nP^3)$     \\
    \bottomrule
  \end{tabular}
    \end{minipage}%
    \begin{minipage}[t]{.4\linewidth}
        \centering
        \caption{Radon models} 
        \label{tab:radon_models}
        \begin{tabular}{ll}
          \toprule
        $M$ & Description \\ 
          \midrule
         1 & Full pooling \\ 
         2 & Partial pooling \\ 
         3 & No pooling \\ 
         4 & Variable intercept \\
         5 & Variable slope \\ 
         6 & Variable intercept and slope \\  
         \bottomrule
        \end{tabular}
    \end{minipage} 
\end{table}

\begin{table}

\end{table}


